MT-R1-Zero: Advancing LLM-based Machine Translation via R1-Zero-like Reinforcement Learning

Large-scale reinforcement learning (RL) methods have proven highly effective in enhancing the reasoning abilities of large language models (LLMs), particularly for tasks with verifiable solutions such as mathematics and coding. However, applying this idea to machine translation (MT), where outputs are flexibly formatted and difficult to automatically evaluate with explicit rules, remains underexplored. In this work, we introduce MT-R1-Zero, the first open-source adaptation of the R1-Zero RL framework for MT without supervised fine-tuning or cold-start. We propose a rule-metric mixed reward mechanism to guide LLMs towards improved translation quality via emergent reasoning. On the WMT 24 English-Chinese benchmark, our MT-R1-Zero-3B-Mix achieves competitive performance, surpassing TowerInstruct-7B-v0.2 by an average of 1.26 points. Meanwhile, our MT-R1-Zero-7B-Mix attains a high average score of 62.25 across all metrics, placing it on par with advanced proprietary models such as GPT-4o and Claude-3.5-Sonnet, while the MT-R1-Zero-7B-Sem variant achieves state-of-the-art scores on semantic metrics. Moreover, our work exhibits strong generalization capabilities on out-of-distribution MT tasks, robustly supporting multilingual and low-resource settings. Extensive analysis of model behavior across different initializations and reward metrics offers pioneering insight into the critical role of reward design, LLM adaptability, training dynamics, and emergent reasoning patterns within the R1-Zero paradigm for MT. Our code is available at https://github.com/fzp0424/MT-R1-Zero.

==> table/redstar_enxx.tex <==
\begin{table*}[htbp]
    \centering
    \setlength{\tabcolsep}{3pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccccccccccccccc}
        \toprule[0.5mm]
        & \multicolumn{2}{c}{EN-AF} & \multicolumn{2}{c}{EN-DA} & \multicolumn{2}{c}{EN-DE} & \multicolumn{2}{c}{EN-IS} 
        & \multicolumn{2}{c}{EN-NL} & \multicolumn{2}{c}{EN-NO} & \multicolumn{2}{c}{EN-SV} & \multicolumn{2}{c}{Avg. EN-XX} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} 
        \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15} \cmidrule(lr){16-17}
        Models & COMET-22 & XCOMET & COMET-22 & XCOMET & COMET-22 & XCOMET & COMET-22 & XCOMET 
        & COMET-22 & XCOMET & COMET-22 & XCOMET & COMET-22 & XCOMET & COMET-22 & XCOMET \\
        \midrule
        LLaMA-3.1-8B-Instruct & 84.8 & 74.5 & 86.6 & 71.7 & 77.5 & 68.8 & 69.4 & 53.6 
        & 81.1 & 72.5 & 85.6 & 74.0 & 80.8 & 67.3 & 80.8 & 68.9 \\
        Aya-101 & 78.8 & 40.8 & 87.6 & 62.9 & 84.3 & 67.5 & 84.3 & 74.5 
        & 85.8 & 72.2 & 87.5 & 69.0 & 86.9 & 61.2 & 85.0 & 64.0 \\
        Aya-23-8B & 79.6 & 68.2 & 76.4 & 56.6 & 88.1 & 77.0 & 38.4 & 9.6 
        & 87.9 & 78.8 & 77.3 & 60.0 & 78.3 & 59.7 & 75.1 & 58.5 \\
        Aya-23-35B & 81.2 & 67.9 & 82.9 & 65.5 & 88.1 & 77.2 & 51.0 & 28.6 
        & 87.9 & 78.2 & 82.4 & 67.6 & 83.7 & 67.9 & 79.6 & 64.7 \\
        X-ALMA & 87.6 & 75.8 & 92.0 & 79.7 & 88.8 & 78.0 & 87.2 & 78.5 
        & 89.0 & 80.4 & 90.8 & 81.5 & 91.8 & 81.0 & 89.6 & 79.3 \\
        MT-R1-Zero (Qwen2.5-7B) & 80.2 & 89.5 & 84.2 & 84.2 & 86.5 & 95.3 & 64.8 & 80.1 
        & 86.3 & 91.2 & 83.2 & 85.1 & 84.6 & 84.2 & 81.4 & 87.1 \\
        MT-R1-Zero (LLaMA-3.1-8B) & 85.4 & 89.9 & 89.7 & 92.9 & 87.6 & 96.6 & 70.9 & 93.9 
        & 87.7 & 94.6 & 89.1 & 93.7 & 90.4 & 93.9 & 85.8 & 93.5 \\
        \bottomrule[0.5mm]
    \end{tabular}
    }
    \caption{Performance comparison of MT-R1-Zero (Multilingual) against other baseline and multilingual models across multiple EN-XX translation directions.}
    \label{tab:red_star}
\end{table*}


==> table/redstar_xxen.tex <==
\begin{table*}[htbp]
    \centering
    \setlength{\tabcolsep}{3pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccccccccccccccc}
        \toprule[0.5mm]
        & \multicolumn{2}{c}{AF-EN} & \multicolumn{2}{c}{DA-EN} & \multicolumn{2}{c}{DE-EN} & \multicolumn{2}{c}{IS-EN} 
        & \multicolumn{2}{c}{NL-EN} & \multicolumn{2}{c}{NO-EN} & \multicolumn{2}{c}{SV-EN} & \multicolumn{2}{c}{Avg. XX-EN} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} 
        \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15} \cmidrule(lr){16-17}
        Models & COMET-22 & XCOMET & COMET-22 & XCOMET & COMET-22 & XCOMET & COMET-22 & XCOMET 
        & COMET-22 & XCOMET & COMET-22 & XCOMET & COMET-22 & XCOMET & COMET-22 & XCOMET \\
        \midrule
        LLaMA-3.1-8B-Instruct & 66.2 & 33.9 & 66.5 & 52.5 & 78.6 & 72.3 & 43.4 & 42.0 
        & 78.7 & 74.5 & 72.7 & 54.1 & 75.5 & 70.5 & 68.8 & 57.1 \\
        Aya-101 & 86.1 & 65.4 & 89.2 & 75.9 & 88.5 & 77.9 & 82.3 & 68.4 
        & 86.9 & 78.3 & 88.1 & 76.0 & 89.4 & 78.5 & 87.2 & 74.4 \\
        Aya-23-8B & 85.3 & 70.6 & 87.7 & 76.8 & 89.3 & 78.9 & 68.0 & 46.5 
        & 87.5 & 79.0 & 86.5 & 75.8 & 87.9 & 76.7 & 84.6 & 72.0 \\
        Aya-23-35B & 89.7 & 74.9 & 89.7 & 79.4 & 89.5 & 78.6 & 78.5 & 66.1 
        & 87.8 & 78.8 & 88.5 & 78.8 & 89.5 & 79.6 & 87.4 & 76.6 \\
        X-ALMA & 90.0 & 76.6 & 90.7 & 80.4 & 89.6 & 79.2 & 87.2 & 76.6 
        & 88.1 & 79.3 & 89.5 & 79.5 & 90.6 & 80.6 & 89.4 & 78.9 \\
        MT-R1-Zero (Qwen2.5-7B) & 88.1 & 89.5 & 89.4 & 96.8 & 86.5 & 95.3 & 76.6 & 80.1 
        & 87.5 & 97.2 & 88.2 & 85.1 & 89.4 & 96.7 & 86.5 & 91.5 \\
        MT-R1-Zero (LLaMA-3.1-8B) & 85.4 & 94.5 & 89.9 & 98.0 & 87.6 & 96.6 & 83.6 & 93.9 
        & 87.7 & 98.0 & 88.9 & 97.6 & 90.0 & 97.8 & 87.6 & 96.6 \\
        \bottomrule[0.5mm]
    \end{tabular}
    }
    \caption{Performance comparison across different language directions. Our MT-R1-Zero model achieves the highest XCOMET scores on all language pairs.}
    \label{tab:red_star}
\end{table*}

